Subgraph Federated Learning for Local Generalization

Federated Learning (FL) on graphs enables collaborative model training to enhance performance without compromising the privacy of each client. However, existing methods often overlook the mutable nature of graph data, which frequently introduces new nodes and leads to shifts in label distribution. Since they focus solely on performing well on each client's local data, they are prone to overfitting to their local distributions (i.e., local overfitting), which hinders their ability to generalize to unseen data with diverse label distributions. In contrast, our proposed method, FedLoG, effectively tackles this issue by mitigating local overfitting. Our model generates global synthetic data by condensing the reliable information from each class representation and its structural information across clients. Using these synthetic data as a training set, we alleviate the local overfitting problem by adaptively generalizing the absent knowledge within each local dataset. This enhances the generalization capabilities of local models, enabling them to handle unseen data effectively. Our model outperforms baselines in our proposed experimental settings, which are designed to measure generalization power to unseen data in practical scenarios. Our code is available at https://github.com/sung-won-kim/FedLoG

==> sections/methodology.tex <==

Our proposed subgraph-FL framework, \proposed, works as follows:
\vspace{-0.4ex}
\begin{itemize}[leftmargin=.1in]
\setlength \itemsep{-0.1ex}
    \item \textbf{Step 1 -- Local Fitting (Section \ref{subsec:localfit}):} 
    The server initializes the local model parameters of \(K\) clients with the parameters of the global model \(\phi\). Each local model is then trained using local data \(\mathcal{D}_k\). Concurrently, \textcolor{orange}{head degree} and tail degree knowledge are condensed into synthetic nodes within each client, denoted as \(\mathcal{V}_{k,\text{head}}\) and \(\mathcal{V}_{k,\text{tail}}\).   
    \item \textbf{Step 2 -- Global Aggregation and Global Synthetic Data Generation (Section \ref{sec:aggregation}):} After local training, the server aggregates the local models to create the global model \(\phi\), and generates global synthetic data \(\mathcal{D}_g\) by aggregating \(\mathcal{V}_{k,\text{head}}\) for all \(k\), weighted by the proportion of the \textcolor{cyan}{head classes} within each client $k$. 
    % Moreover, synthetic data \(\mathcal{D}_g\) is supplemented with neighboring information with aggregated local neighbor generators.
    % \item \textbf{Step 2 -- Global Aggregation and Global Synthetic Data Generation (Section \ref{sec:aggregation}):} After local training, the server aggregates the local models to create the global model \(\phi\), and generates global synthetic data \(\mathcal{D}_g\) by aggregating \(\mathcal{V}_{k,\text{head}}\) for all \(k\), with unbiased neighbor generator. 
    \item \textbf{Step 3 -- Local Fitting (Section \ref{subsec:localfit}) \& Local Generalization (Section \ref{subsec:localgen}):} Similar to Step 1, local fitting and data condensation proceed. After local fitting, local models are generalized using \(\mathcal{D}_g\) which possess both \textcolor{orange}{head degree} and \textcolor{cyan}{head class} knowledge, adaptively learning the locally absent knowledge. 
\end{itemize}
\vspace{-0.4ex}
While the framework starts with Step 1, it continues to alternate between Steps 2 and 3 until the final round \(R\) is reached.  
In summary, our method extracts \textcolor{orange}{head degree} knowledge at the \textcolor{orange}{client} level and \textcolor{cyan}{head class} knowledge at the \textcolor{cyan}{server} level, then condense them into the global synthetic data,
which is utilized to train the local model during Local Generalization to adaptively compensate for the locally absent knowledge within each client.
The overall framework of \proposed~is depicted in Figure \ref{fig:archi}, and its algorithm is described in Algorithm~\ref{alg:pseudo}.

\vspace{-1ex}
\subsection{Local Fitting}
\label{subsec:localfit}
\vspace{-0.5ex}

The local model for each client $k$ consists of one GNN embedder (\(\varphi_{k,E}\)) and two classifiers (\(\varphi_{k,H}\) and \(\varphi_{k,T}\)), for the head and tail degree branches, respectively, as shown in Figure \ref{fig:archi}(b1). 
Each branch has \(s \times |\mathcal{C}_\mathcal{V}|\) learnable nodes, each with features of dimension \(d\), allocating \(s\) nodes per class. Thus, each client has learnable node sets \(\mathcal{V}_{k,\text{head}}\) and \(\mathcal{V}_{k,\text{tail}}\) with features \(X_{\mathcal{V}_{k,\text{head}}}\in \mathbb{R}^{(s \times |\mathcal{C}_\mathcal{V}|) \times d}\) and \(X_{\mathcal{V}_{k,\text{tail}}} \in \mathbb{R}^{(s \times |\mathcal{C}_\mathcal{V}|) \times d}\), respectively.
At the client level, we condense knowledge from locally observed nodes into these learnable nodes. 
Head degree nodes are condensed into \(\mathcal{V}_{k,\text{head}}\) and tail degree nodes into \(\mathcal{V}_{k,\text{tail}}\), integrating condensation and prediction into a single process. 
Learnable nodes serve as prototypes within each branch, forming a prototypical network. The detailed processes are as follows:

\begin{figure}[t] %%% t: top, b: bottom, h: here
\begin{center}
\includegraphics[width=0.93\linewidth]{figures/architecture2.pdf}
\end{center}
\vspace{-1.2em}
\caption{Overview of \proposed~with 2 Clients and 3 Classes.}
\vspace{-1.5em}
\label{fig:archi}
\end{figure}

\textbf{(Initialization)} In the initial round ($r = 0$), we initialize the local model weights for each client \(k\), denoted as \(\phi_k = \{\varphi_{k,E}, \varphi_{k,H}, \varphi_{k,T}\}\), with the global set of parameters \(\phi = \{\varphi_E, \varphi_H, \varphi_T\}\).

\textbf{(Embedding)} 
For each node \(v_k \in \mathcal{V}_k\) with initial features \(h_{v_k}^{(0)} = x_{v_k}\), 
% a GNN embedder \(\varphi_{k,E}\), an \(L\)-layer GraphSAGE \cite{graphsage}, 
a shared GraphSAGE \cite{graphsage} GNN encoder \(\varphi_{k,E}\) is employed to embed the local node \(v_k \in \mathcal{V}_k\) and the learnable nodes \(v_{k,\text{head}} \in \mathcal{V}_{k,\text{head}}\) and \(v_{k,\text{tail}} \in \mathcal{V}_{k,\text{tail}}\):
\begin{equation}
\label{eq:gnn}
\small
h_{v_k} = \textbf{GNN}_{\varphi_{k,E}}(v_k, \mathcal{G}_k), \quad h_{v_{k,\text{head}}} = \textbf{GNN}_{\varphi_{k,E}}(v_{k,\text{head}}, \mathcal{G}_I), \quad h_{v_{k,\text{tail}}} = \textbf{GNN}_{\varphi_{k,E}}(v_{k,\text{tail}}, \mathcal{G}_I)
\end{equation}
where \(h_{v_k}\), \(h_{v_{k,\text{head}}}\), and \(h_{v_{k,\text{tail}}}\) are the representations of nodes \(v_k\), \(v_{k,\text{head}}\), and \(v_{k,\text{tail}}\), respectively, and \(\mathcal{G}_I\) represents a discrete graph with no edges. 
The learnable nodes do not adhere to a specific graph structure but share the same GNN encoder with the local graph, allowing us to condense structural information into the features of the learnable nodes.

After acquiring node representations, we generate model predictions in each branch using class prototypes, which are the representations of learnable nodes.
% We use the representations of learnable nodes as class prototypes for each branch.
For instance, in the head branch, prototypes are defined as \(P_{k,\text{head}} = \{h_{v_{k,\text{head}}^{(1,1)}}, \ldots, h_{v_{k,\text{head}}^{(1,s)}}, \ldots, h_{v_{k,\text{head}}^{(|\mathcal{C_V}|,1)}}, \ldots, h_{v_{k,\text{head}}^{(|\mathcal{C_V}|,s)}}\}\), with \(s\) prototypes per class.
To ensure all class information contributes to the final prediction, the target node representations are further updated based on feature differences with all prototypes assigned to each class as follows: $h_{v_k}' = \varphi_{k,H}(h_{v_k}, \{h_{v_k}-h_{v_{k,\text{head}}^{(1,1)}}, \ldots, h_{v_k}-h_{v_{k,\text{head}}^{(|\mathcal{C_V}|,s)}}\})$.
Please refer to Appendix~\ref{apx:classifier} for more details on \(\varphi_{k,H}\).
Then, the class probability for target node $v_k$ is given as follows:
\begin{equation}
\small
\label{eq:classifier}
p(c | h_{v_k}') = \frac{\exp(-d(h_{v_k}', \bar{h}_{\mathcal{V}_{k,\text{head}}^c}))}{\sum_{c'=1}^{|\mathcal{C_V}|} \exp(-d(h_{v_i}', \bar{h}_{\mathcal{V}_{(k,\text{head})}^{c'}}))},
\end{equation}
where \(d(\cdot,\cdot)\) is the squared Euclidean distance and 
\(\bar{h}_{\mathcal{V}_{k,\text{head}}^c}\) indicates the average of prototype representations of class $c$, i.e., \(\bar{h}_{\mathcal{V}_{k,\text{head}}^c} = \frac{1}{s} \sum_{i=1}^s h_{v_{k,\text{head}}^{(c,i)}}\).

% \begin{equation}
% \label{eq:classifier}
% h_{v_i}' = \varphi_{k,H}(h_{v_i}, \{h_{v_i}-h_{v_{\text{head},1}^{1}}, \ldots, h_{v_i}-h_{v_{\text{head},s}^{|\mathcal{C_V}|}}\}),
% \end{equation}
% where the class probability for target node \(v_i\) is
% % \begin{equation}
% $p(c | h_{v_i}') = \frac{\exp(-d(h_{v_i}', \bar{h}^c_{\text{head}}))}{\sum_{c'=1}^{|\mathcal{C_V}|} \exp(-d(h_{v_i}', \bar{h}^{c'}_{\text{head}}))}$,
% % \end{equation}
% with \(d(\cdot,\cdot)\) as the squared Euclidean distance and \(\bar{h}^c_{\text{head}} = \frac{1}{s} \sum_{i=1}^s h_{v_{\text{head},i}^{c}}\). See Appendix~\ref{apx:classifier} for more details on \(\varphi_{k,H}\).


To obtain final prediction \(\mathrm{\textbf{p}}\) , we combine the class probabilities from both branches \(\mathrm{\textbf{p}}_{\text{head}}\) and \(\mathrm{\textbf{p}}_{\text{tail}}\) by weighting them based on the degree value of the target node \(v_k\) (i.e., $\text{deg}(v_k)$) as follows:
\begin{equation}
    \mathrm{\textbf{p}} = \alpha \cdot \mathrm{\textbf{p}}_{\text{head}} + (1 - \alpha) \cdot \mathrm{\textbf{p}}_{\text{tail}},
\label{eq:brch_merge}
\end{equation}
where $\alpha = 1/(1 + e^{- (\text{deg}(v_k) - (\lambda + 1))})$, 
and \(\lambda\) is the tail degree threshold outlined in the Appendix~\ref{apx:tail_thres}.
Note that, the parameter \(\alpha\) balances the influence of head and tail branches based on the node's degree, preventing nodes with very high degree from dominating the head branch.
High-degree nodes, which rely heavily on the head degree branch for predictions, significantly influence the features of learnable nodes within the head degree branch, condensing their knowledge into \(\mathcal{V}_{k,\text{head}}\). 
The tail degree branch specializes in classifying tail-degree nodes, which possess knowledge that is not suitable for sharing across clients due to their potentially noisy characteristics \cite{degreebias, liu2021tail, wu2021self, xiao2021learning}.
Then, the prediction loss for each client $k$ is calculated as follows:
% \begin{equation}
$\mathcal{L}_{k,cls} = \sum_{v_k \in \mathcal{V}_k} \sum_{c \in \mathcal{C_V}} -\mathbb{I}(y_{v_k} = c) \log(\mathrm{\textbf{p}}[c]) \label{eq:prediction_loss}$.
% \end{equation}

% Finally, we optimize the model parameters \(\phi_k\) and update the learnable nodes' features using the prediction loss \(\mathcal{L}_{k,cls}\). 
Furthermore, to ensure the stability of the condensation process, we minimize the \(L_2\) norm of the learnable features, denoted as \(\mathcal{L}_{k,norm}\). 
Thus, the total loss for model parameters is \(\mathcal{L}_k(\phi_k, X_{\mathcal{V}_{k,\text{head}}}, X_{\mathcal{V}_{k,\text{tail}}}) = \mathcal{L}_{k,cls} + \beta \cdot \mathcal{L}_{k,norm}\), where \(\beta\) adjusts the extent of regularization.






\subsection{Global Aggregation and Global Synthetic Data Generation}
\label{sec:aggregation}


 

\textbf{Global Aggregation.}
After training the $K$ local clients, the server aggregates the local model weights for round \(r\) using the weighted average 
$\phi^{(r+1)} \leftarrow \frac{1}{K} \sum_{k=1}^K \phi_k^{(r)}$.

\textbf{Global Synthetic Data Generation.}
% \textbf{Initial Node Feature Generation.}
In addition, the server generates global synthetic data, which will be employed during the Local Generalization phase (Section \ref{subsec:localgen}) to help mitigate the issue of local overfitting.
More specifically, we first generate node features in global synthetic data \(\mathcal{D}_g\) by merging the \textcolor{orange}{head degree} condensed nodes \(\mathcal{V}_{k,\text{head}}\) from all clients, weighted by the proportion of \textcolor{cyan}{head classes} for each client, 
since each client has expert knowledge of the dominant classes within their data as shown in Section~\ref{sec:reliable}. 
% The server then generates global synthetic data \(\mathcal{D}_g\) by merging the \textcolor{orange}{head degree} condensed nodes \(\mathcal{V}_{k,\text{head}}\) from all clients, weighted by the proportion of \textcolor{cyan}{head classes} for each client. 
% Each client is assumed to have expert knowledge of the dominant classes within their data.
% In Figure~\ref{fig:archi}(d), for each class \(c \in \mathcal{C}\), the feature vector of the \(i\)-th global synthetic node for class \(c\), \(x_{g,i}^c\), is defined as:
% $x_{g,i}^c = \frac{1}{\sum_{k=1}^K r_{k}^{c}} \sum_{k=1}^K r_{k}^{c} x_{k,v_{\text{head},i}^{c}}$,
% where \(r_{k}^{c} = \frac{|\mathcal{V}_{k}^{c}|}{|\mathcal{V}_k|}\) represents the proportion of nodes labeled \(c\) in the \(k\)-th client's dataset.
% The server generates \(s \times |\mathcal{C_V}|\) global synthetic nodes \(\mathcal{V}_{g}\) with features \(X_g=\{x_{g,1}^1, \ldots, x_{g,s}^1, \ldots, x_{g,1}^{|\mathcal{C_V}|}, \ldots, x_{g,s}^{|\mathcal{C_V}|}\}\), encompassing knowledge related to both head degree and head class across clients. 
% Thus, the initially generated global synthetic data is \(\mathcal{D}_g = (\mathcal{G}_g = (\mathcal{V}_g, \mathcal{E}_\varnothing), Y_{\mathcal{V}_g})\).
% As shown in Section~\ref{sec:reliable}, each client has expert knowledge of the dominant classes within local data
More formally, for each class \(c \in \mathcal{C}\), the feature vector of the \(i\)-th global synthetic node for class \(c\), \(x_{v_{g}^{(c,i)}}\), is generated as follows:
% In Figure~\ref{fig:archi}(d), for each class \(c \in \mathcal{C}\), the feature vector of the \(i\)-th global synthetic node for class \(c\), \(x_{v_{g}^{(c,i)}}\), is generated as:
\vspace{-2ex}
\begin{equation}\label{eq:global_syn_gen}
\small
x_{v_{g}^{(c,i)}} = \frac{1}{\sum_{k=1}^K r_{k}^{c}} \sum_{k=1}^K r_{k}^{c} x_{v_{k,\text{head}}^{(c,i)}},
\end{equation}
where \(r_{k}^{c} = \frac{|\mathcal{V}_{k}^{c}|}{|\mathcal{V}_k|}\) represents the proportion of nodes labeled \(c\) in the \(k\)-th client's dataset.
In this way, the server generates \(s \times |\mathcal{C_V}|\) global synthetic nodes \(\mathcal{V}_{g}\) with features \(X_{\mathcal{V}_g}=\{x_{v_{g}^{(1,1)}}, \ldots, x_{v_{g}^{(1,s)}}, \ldots, x_{v_{g}^{(|\mathcal{C_V}|,1)}}, \ldots, x_{v_{g}^{(|\mathcal{C_V}|,s)}}\}\), encompassing knowledge related to both head degree and head class across clients. Thus, the initially generated global synthetic data is \(\mathcal{D}_g = (\mathcal{G}_g = (\mathcal{V}_g, \mathcal{E}_\varnothing), Y_{\mathcal{V}_g})\) with node features $X_{\mathcal{V}_g}$.



% \textbf{Unbiased Neighbor Generation.}
Although structural information is vital for understanding the data distribution in graph-structured data, the initially generated global synthetic data \(\mathcal{D}_g\) comprises only the feature information of nodes and lacks any surrounding neighbor information. 
% Therefore, we propose to generate a single neighbor node, which can effectively represent $h$-hop subgraph of the synthetic node, with pre-trained neighbor generators, which are specially trained to generate class-specific neighbors.
Consequently, we propose generating a single neighbor node that can effectively represent the $h$-hop subgraph of the synthetic node, using pre-trained neighbor generators. 
These generators are specifically trained to produce class-specific neighbors, as elaborated in Section \ref{subsec:neighgen}.
% Therefore, we propose generating neighborhoods for the synthetic nodes with pre-trained neighbor generators, which are specially trained to generate class-specific neighbors. 
% The pre-training process is elaborated in Section \ref{subsec:neighgen}.
Local clients utilize these neighbor generators at the local level to adaptively customize the features of the global synthetic data, and then generate the neighbors of the customized features, as detailed in following Section~\ref{subsec:localgen}.

In summary, at the end of each round \(r\), the server distributes the aggregated model weights \(\phi^{(r+1)}\) and the generated global synthetic data \(\mathcal{D}_g\).

% Briefly speaking, we pre-train the neighbor generator for each client to generate neighbors of the target node within the local graph. Since each client has a different label distribution, the pre-trained neighbor generator tends to be biased towards generating the dominant class within its local data. To alleviate this, we aggregate these local neighbor generators in a class-wise manner at the server so that each neighbor generator has expert knowledge of its assigned class.
% \textcolor{red}{Finally, How to aggregate generated neighbors and initinial node feature?}


\subsection{Local Generalization}

% \subsection{Step 3 -- Local Fitting \& Local Generalization (Round $r>1$)} 
\label{subsec:localgen}
At the beginning of each round (\(r > 1\)), each client initializes its local model with the distributed global model parameters \(\phi\). 
After the local update within their local data (i.e., Local Fitting), we additionally train the local model with the global synthetic data \(\mathcal{D}_g\), enabling it to generalize to locally absent knowledge (i.e., Local Generalization), such as tail and missing classes.
% This approach helps prevent the local overfitting problem. 
Since each client has different locally absent knowledge, we first adaptively customize the global synthetic data for the current state of local model and then train with the customized data.


% \textbf{Local Adaptation -- Feature Scaling.} In order to adaptively customize the global synthetic data, we use feature scaling of the global data \(X_g=\{x_{g,1}^1, \ldots, x_{g,s}^1, \ldots, x_{g,1}^{|\mathcal{C_V}|}, \ldots, x_{g,s}^{|\mathcal{C_V}|}\}\) as follows:
% \begin{equation}
% \hat{x}_{g,i}^c = x_{g,i}^c + \gamma_k[c]\cdot(\bar{x}_{g} - x_{g,i}^c), \text{ where }\bar{x}_g = \frac{1}{\left\vert\mathcal{V}_g\right\vert} \sum_{x\in X_g} x,
% \end{equation}
% where \(\gamma_k \in \mathbb{R}^{|\mathcal{C_V}|}\) denotes the adaptive factor which adjust the difficulty of predictions for the training data on a class-wise basis.
% The elements of adaptive factor $\gamma_k[c]$ for corresponding class $c$ is increased by 0.001 at the end of the round, when the local model's accuracy for class $c$ within global synthetic nodes $\mathcal{V}_g$ above the threshold.
% We initialize the elements of \(\gamma_k\) to 0 in the first round.

% More specifically, if the local model has good predictions for class \(c\) (i.e., class accuracy above the threshold), we scale the global synthetic data for class \(c\) to be closer to the decision boundary, making it harder to predict. 
% This reduces the weight norm for the major classes, preventing overfitting to the head class \cite{cuda}, while the model can learn minority and missing classes step-by-step, similar to curriculum learning [cites CL].
% We approximately assume that a decision boundary for all classes is the mean of all prototypes (i.e., $\bar{x}_g$).


\textbf{Local Adaptation -- Feature Scaling.} 
Motivated by recent work \cite{cuda}, we adjust the difficulty of the training data class-wise to prevent overfitting to major classes while allowing the model to effectively learn tail and missing classes. To achieve this, we use feature scaling on the global synthetic data \(X_{\mathcal{V}_g} = \{x_{v_{g}^{(1,1)}}, \ldots, x_{v_{g}^{(1,s)}}, \ldots, x_{v_{g}^{(|\mathcal{C_V}|,1)}}, \ldots, x_{v_{g}^{(|\mathcal{C_V}|,s)}}\}\) as follows:
\vspace{-1ex}
\begin{equation} \label{eq:feature_scale}
\small
\hat{x}_{v_{g}^{(c,i)}} = x_{v_{g}^{(c,i)}} + \gamma_k[c] \cdot (\bar{x}_{\mathcal{V}_g} - x_{v_{g}^{(c,i)}}), \text{ where } \bar{x}_{\mathcal{V}_g} = \frac{1}{\left\vert \mathcal{V}_g \right\vert} \sum_{x_{v_g} \in X_{\mathcal{V}_g}} x_{v_g},
\end{equation}  
\vspace{-2.5ex}

where \(\gamma_k \in \mathbb{R}^{|\mathcal{C_V}|}\) is a class-wise adaptive factor that adjusts prediction difficulty by moving the global synthetic data of class $c$ to the average of global synthetic data, making it harder to predict. 
Note that when \(\gamma_k = 1\), the global synthetic data for class $c$ is completely replaced with the average of the global synthetic data, whereas the global synthetic data for class $c$ remains unchanged when \(\gamma_k = 0\).
During training, we dynamically modify the factor by incrementing it by 0.001 whenever the local model’s accuracy for class $c$ exceeds the threshold at the end of the round, thereby increasing the difficulty of the corresponding class.
% The decision boundary is approximated as the mean of all prototypes (\(\bar{x}_{\mathcal{V}_g}\)). 
% We initialize \(\gamma_k\) to 0 in the first round. If the local model's accuracy for class \(c\) is above the threshold at the end of the round, \(\gamma_k[c]\) is increased by 0.001, thereby increasing the difficulty of the corresponding class.

\textbf{Local Adaptation -- Neighbor Generation.}
As structural information is crucial for optimizing the GNN model, we generate a neighbor for each customized global synthetic data using the class-specific neighbor generator \(\mathbf{NG}^c\) for the corresponding class \(c\), as shown in Figure~\ref{fig:archi}(b2). We then construct the synthetic graph set \({\mathcal{G}}_{k}^{\text{syn}}\), which consists of graphs, each containing the customized global synthetic node neighboring with its generated neighbor node. It is worth noting that the generated neighbor node effectively represents the $h$-hop subgraph structure of each synthetic node. The details of how to pre-train the neighbor generators are provided in Section~\ref{subsec:neighgen}.



\noindent \textbf{Train with Customized Data.}
Using the synthetic graphs \({\mathcal{G}}_{k}^{\text{syn}}\), the prediction for the target synthetic nodes within $\mathcal{V}_g$ follows Eqs.~\ref{eq:gnn}-\ref{eq:brch_merge} using the same local model $\phi_k$ as for normal nodes $\mathcal{V}_k$, with \(\alpha\) set to 0.5.
The prediction loss for \(\mathcal{D}_g\) is 
$\mathcal{L}_{k,g} = \sum_{v_g \in \mathcal{V}_g} \sum_{c \in \mathcal{C}_{\mathcal{V}}} -\mathbb{I}(y_{v_g} = c) \log(\mathrm{\textbf{p}}[c])$.
At the end of each round, we adjust the adaptive factor \(\gamma_k\) based on the class prediction accuracy. 

In summary, the final loss of the local model is:
$\mathcal{L}_k = \mathcal{L}_{k,cls} + \mathcal{L}_{k,g}$.

\vspace{-1ex}
\subsection{Pretrain Neighbor Generators} 
\label{subsec:neighgen}
\vspace{-1.2ex}

In this section, we will conceptually outline the process of pretraining local neighbor generators and the method of aggregating these generators on the server to produce unbiased local neighbors. 
A detailed description of this process can be found in Appendix~\ref{apx:neighgen}.


% In this section, we will conceptually describe the pretraining process; the detailed process is explained in Appendix~\ref{apx:neighgen}.
% Overall, we pre-train the neighbor generators within each client to capture the client-specific label distributions, then we aggregate these local neighbor generators on a class-wise manner in server. 
% This approach allows the global neighbor generators to learn the comprehensive distribution rather than a distribution that is biased locally.

\paragraph{Training Local Neighbor Generators.} In Figure~\ref{fig:archi}(a), we train a neighbor generator \(\mathbf{NG}_k\) for each local client \(k\). 
Let \({\mathcal{G}}_{k,v_{k}}^{\text{syn}}\) be the generated synthetic graph consisting only of the target node \(v_k\) and the generated neighbor node \(\mathcal{N}_{v_k}\).
Our goal is to condense \cite{jin2021graph, jin2022condensing} the true \(h\)-hop subgraph of the target node \(v_k\), denoted as \(\mathcal{G}_{k,v_k}\), into the synthetic graph \({\mathcal{G}}_{k,v_k}^{\text{syn}}\).
We achieve this by condensing the feature information of \(h\)-hop neighbor nodes through feature matching between the generated neighbor feature and the mean of true \(h\)-hop node features (i.e., $\mathcal{L}_{k,\text{feat}}$). 
The input is the feature vector \(x_{v_k}\), producing a neighbor feature \(\hat{x}_{\mathcal{N}_{v_k}} = \mathbf{NG}_k(x_{v_k})\). 
Additionally, to align with the training mechanism of GNNs, we closely mimic the effects of the gradients by gradient matching. This involves minimizing the difference between gradients for predicting the target node using \(\mathcal{G}_{k,v_k}\) and \({\mathcal{G}}_{k,v_k}^{\text{syn}}\), respectively, utilizing the same GNNs (i.e., $\mathcal{L}_{k,\text{grad}}$).
The loss function for training the local neighbor generator $\mathbf{NG}_k$ is $\mathcal{L}_{\mathbf{NG}_k} = \mathcal{L}_{k,\text{feat}} + \mathcal{L}_{k,\text{grad}}$.

\paragraph{Aggregate Neighbor Generators in Server.} 
Since clients have different label distributions, local neighbor generators are biased towards generating neighbors for dominant classes within their local graphs. Hence, we aggregate these generators in a class-wise manner, as depicted in Figure~\ref{fig:archi}(a).
This can be formulated as 
% \begin{equation}
$\mathbf{NG}^c = \frac{1}{\sum_{k=1}^K r_{k}^{c}} \sum_{k=1}^K r_{k}^{c} \mathbf{NG}_k$,
% \end{equation}
where \(r_{k}^{c} = \frac{|\mathcal{V}_{k}^{c}|}{|\mathcal{V}_k|}\) represents the proportion of nodes with label \(c\) in the \(k\)-th client’s dataset. These class-specific neighbor generators \(\mathbf{NG}^c\) for all \(c\) are then frozen and shared with all clients for the federated learning process to generate the synthetic graph for global synthetic data \(\mathcal{D}_g\) that is not locally biased as described in Section \ref{subsec:localgen}.


==> tables/tab2_fig3.tex <==
\begin{wrapfigure}{r}{0.35\textwidth} % Adjust the width as needed
    \vspace{-0.8ex} % Adjust vertical space as needed
    \begin{minipage}{0.35\textwidth}
        \centering
        \captionsetup{type=table}
        \caption{\(\gamma[c]\) values at round $R$ (CiteSeer - 3 Clients).}
        \vspace{-1.5ex}
        \scriptsize % Reduce font size
        \setlength{\tabcolsep}{0pt} 
        \renewcommand{\arraystretch}{0.5} % Adjust row spacing
        \begin{tabularx}{\textwidth}{@{}c*{6}{>{\centering\arraybackslash}X}@{}} % Force table to fit in the specified width
            \cmidrule[1.2pt]{1-7}
            \textbf{Class} & \textbf{1} & \textbf{2} & \textbf{3} & \textbf{4} & \textbf{5} & \textbf{6} \\
            \cmidrule[0.7pt]{1-7}
            \# Nodes & 5 & 27 & \textcolor{red}{\textbf{129}} & 16 & \textcolor{blue}{\textbf{0}} & 25 \\ \cmidrule[0.5pt]{1-7}
            \rowcolor{gray!20} 
            $\gamma[c]$ & 0.288 & 0.289 & \textcolor{red}{\textbf{0.297}} & 0.282 & \textcolor{blue}{\textbf{0.282}} & 0.286 \\
            \cmidrule[1.2pt]{1-7}
        \end{tabularx}
        % \vspace{-6pt}
        % \captionsetup{type=table}
        % \caption{\(\gamma[c]\) values at round $R$ (CiteSeer - 3 Clients).}
        \label{tbl:gamma_value}
        \vspace{3pt}

        \includegraphics[width=1.0\textwidth]{./figures/ablation_class_compact.pdf}
        \captionsetup{type=figure}
        \vspace{-2.5ex}
        % \vspace{-8pt}
        \caption{Ablation Studies (CiteSeer - 3 Clients).} \label{fig:ablation_cls}
        \vspace{-2ex}
    \end{minipage}
\end{wrapfigure}
